Attention as Activation

Activation functions and attention mechanisms are typically treated as having different purposes and have evolved differently. However, both concepts can be formulated as a non-linear gating function. Inspired by their similarity, we propose a novel type of activation units called attentional activation (ATAC) units as a unification of activation functions and attention mechanisms. In particular, we propose a local channel attention module for the simultaneous non-linear activation and element-wise feature refinement, which locally aggregates point-wise cross-channel feature contexts. By replacing the well-known rectified linear units by such ATAC units in convolutional networks, we can construct fully attentional networks that perform significantly better with a modest number of additional parameters. We conducted detailed ablation studies on the ATAC units using several host networks with varying network depths to empirically verify the effectiveness and efficiency of the units. Furthermore, we compared the performance of the ATAC units against existing activation functions as well as other attention mechanisms on the CIFAR-10, CIFAR-100, and ImageNet datasets. Our experimental results show that networks constructed with the proposed ATAC units generally yield performance gains over their competitors given a comparable number of parameters.

==> tabs/tab_ablation.tex <==
% !TEX root = ../root.tex
%\bibliography{../RefBib/refs}

\noindent
\begin{minipage}[t]{.6\textwidth}
\setlength{\tabcolsep}{2.5pt}
\begin{table*}[htbp]
\begin{center}
\caption{Classification accuracy of different aggregation strategies on \textbf{CIFAR-100} with various network depths (b) and widths (c).}
\label{Tab:CIFAR100Aggregation}
% \footnotesize
% \small
\begin{tabular}{c c c c c c c c c c c} 
\toprule  
Scale       & \multicolumn{5}{c}{CIFAR-10}                & \multicolumn{5}{c}{CIFAR-100} \\ 
                    \cmidrule(lr){2-6}                           \cmidrule(lr){7-11}
                  & $b=1$           & $b=2$           & $b=3$          & $b=4$  & $b=5$ & $b=1$           & $b=2$           & $b=3$ & $b=4$ & $b=5$ \\ 
\midrule
GlobalChaATAC  & 0.548          & 0.601          & 0.613          & 0.622          & 0.627          & 0.388          & 0.432          & 0.452          & 0.456          & 0.462 \\
ChaNiN         & 0.893          & 0.917          & 0.922          & 0.926          & 0.929          & 0.743          & 0.776          & 0.792          & 0.796          & 0.801 \\
LocalSENet     & 0.906          & 0.926          & 0.931          & 0.937          & 0.939          & 0.762          & 0.794          & 0.805          & 0.811          & 0.817 \\
ChaATAC (\textit{\textbf{ours}}) & \textbf{0.906} & \textbf{0.927} & \textbf{0.936} & \textbf{0.939} & \textbf{0.940} & \textbf{0.764} & \textbf{0.796} & \textbf{0.812} & \textbf{0.821} & \textbf{0.824} \\
% \midrule[\heavyrulewidth]
% \multicolumn{7}{l}{\footnotesize$^*$ Values differing by less than 0.001 are considered the same due to limited trials.} \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-.5em}
\end{table*}
\end{minipage}% <---------------- Note the use of "%"
\begin{minipage}[t]{.4\textwidth}
\setlength{\tabcolsep}{2pt}
\begin{table}[h]
\begin{center}
\caption{Classification comparison on ImageNet with other state-of-the-art networks}
\label{Tab:ImageNet}\vspace{-.125cm}
% \footnotesize
\small
\begin{tabular}{Sc Sl Sc Sc Sc} 
\toprule  
Architecture                                & GFlops & Params & top-1 err.              & top-5 err. \\
\midrule 
ResNet50   \cite{CVPR16ResNetV1}            & 3.86   & 25.6M  & 22.29                   & 6.18 \\
SE-ResNet50 \cite{CVPR18SENet}            & 3.87   & 28.1M  & 22.12                   & 5.99 \\
AA-ResNet50 \cite{ICCV19AugmentedConv}      & 8.3    & 25.8M  & 22.30                   & 6.20 \\
FA-ResNet50 \cite{NIPS19AttentionConv}      & 7.2    & 18.0M  & 22.40                   & /    \\
GE-$\theta^{+}$-ResNet50 \cite{NIPS18GENet} & 3.87   & 33.7M  & 21.88                   & 5.80 \\
% AFF-ResNet50 (\textbf{\textit{ours}})       & 4.3    & 30.3M  & \textit{\textbf{21.61}} & 5.92 \\
\bottomrule
\end{tabular}
\end{center}\vspace{-.5cm}
\end{table}
\end{minipage}





% \setlength{\tabcolsep}{2.5pt}
% \begin{table*}[htbp]
% \begin{center}
% \caption{Classification accuracy of different aggregation strategies on \textbf{CIFAR-100} with various network depths (b) and widths (c).}
% \label{Tab:CIFAR100Aggregation}
% % \footnotesize
% % \small
% \begin{tabular}{c c c c c c c c c c c} 
% \toprule  
% Dataset                    & Method         & $b=1$ & $b=2$ & $b=3$ & $b=4$ & $b=5$ \\
% \multirow{4}{*}{CIFAR-100} & Global-ChaATAC & 0.548 & 0.601 & 0.613 & 0.622 & 0.627  \\
% Local-ChaNiN         & 0.893 & 0.917 & 0.922 & 0.926 & 0.929 \\
% RefineSE
% & \multicolumn{5}{c}{CIFAR-10}                & \multicolumn{5}{c}{CIFAR-100} \\ 
%                     \cmidrule(lr){2-6}                           \cmidrule(lr){7-11}
%                   & $b=1$           & $b=2$           & $b=3$          & $b=4$  & $b=5$ & $b=1$           & $b=2$           & $b=3$ & $b=4$ & $b=5$ \\ 
% \midrule
% Global-ChaATAC       & 0.548 & 0.601 & 0.613 & 0.622 & 0.627 & 0.388 & 0.432 & 0.452 & 0.456 & 0.462 \\
% Local-ChaNiN         & 0.893 & 0.917 & 0.922 & 0.926 & 0.929 & 0.743 & 0.776 & 0.792 & 0.796 & 0.801 \\
% Local-ChaATAC (ours) & \textbf{0.906} & \textbf{0.927} & \textbf{0.936} & \textbf{0.939} & \textbf{0.940} & \textbf{0.764} & \textbf{0.796} & \textbf{0.812} & \textbf{0.821} & \textbf{0.823} \\
% % \midrule[\heavyrulewidth]
% % \multicolumn{7}{l}{\footnotesize$^*$ Values differing by less than 0.001 are considered the same due to limited trials.} \\
% \bottomrule
% \end{tabular}
% \end{center}
% \vspace{-.5em}
% \end{table*}
